Representational Continuity for Unsupervised Continual Learning

Continual learning (CL) aims to learn a sequence of tasks without forgetting the previously acquired knowledge. However, recent CL advances are restricted to supervised continual learning (SCL) scenarios. Consequently, they are not scalable to real-world applications where the data distribution is often biased and unannotated. In this work, we focus on unsupervised continual learning (UCL), where we learn the feature representations on an unlabelled sequence of tasks and show that reliance on annotated data is not necessary for continual learning. We conduct a systematic study analyzing the learned feature representations and show that unsupervised visual representations are surprisingly more robust to catastrophic forgetting, consistently achieve better performance, and generalize better to out-of-distribution tasks than SCL. Furthermore, we find that UCL achieves a smoother loss landscape through qualitative analysis of the learned representations and learns meaningful feature representations. Additionally, we propose Lifelong Unsupervised Mixup (LUMP), a simple yet effective technique that interpolates between the current task and previous tasks' instances to alleviate catastrophic forgetting for unsupervised representations.

==> figures/5_figure_2.tex <==
\begin{table*}[t!]
\small
\begin{minipage}[t!]{\linewidth}
\includegraphics[width=0.3\textwidth]{figures/images/unsup_interpolation.png}
% \subcaption[]{Interpolation between two unsupervised models.}
\includegraphics[width=0.3\textwidth]{figures/images/sup_interpolation.png}
% \subcaption[]{Interpolation between two supervised models.}
\includegraphics[width=0.3\textwidth]{figures/images/unsup=>sup_interpolation.png}
\end{minipage}
\captionof{figure}{\small {\bf Left:} Interpolation between two unsupervised models. {\bf Middle:} Interpolation between two supervised models. {\bf Right:} Interpolation between unsupervised and supervised models.}
\vspace{-0.15in}
\end{table*}



==> figures/A_feature_maps_tinyimg.tex <==
\begin{figure*}[t!]
\small
\begin{minipage}[t]{1.05\linewidth}
\resizebox{\linewidth}{!}{%
\begin{tabular}{c cccc ccc}
\hspace{-0.2in}
\rb{\includegraphics[width=0.13\textwidth]{figures/tinyimg_feat_maps/T0_imaig0_raw_cropped.PNG}}&
\includegraphics[width=0.17\textwidth]{figures/tinyimg_feat_maps/sup_finetune_3_tiny__T0_imgid0_atT19.png} & \hspace{-0.3in}
\includegraphics[width=0.17\textwidth]{figures/tinyimg_feat_maps/sup_si_1_tinyimg__T0_imgid0_atT19.png} & \hspace{-0.3in}
\includegraphics[width=0.17\textwidth]{figures/tinyimg_feat_maps/sup_gss_3__T0_imgid0_atT19.png} & \hspace{-0.3in}
\includegraphics[width=0.17\textwidth]{figures/tinyimg_feat_maps/sup_der_3_tinyimg__T0_imgid0_atT19.png} & \hspace{-0.2in}
\includegraphics[width=0.17\textwidth]{figures/tinyimg_feat_maps/unsup_finetune_1_tinyimg__T0_imgid0_atT19.png} & \hspace{-0.3in}
\includegraphics[width=0.17\textwidth]{tbd.png} & \hspace{-0.3in}
\includegraphics[width=0.17\textwidth]{figures/tinyimg_feat_maps/unsup_mixup_3_0.4_tiny__T0_imgid0_atT19.png} \vspace{-0.1in}\\
\hspace{-0.2in} \textsc{Phone} ($t_0$) & \specialcell{\textsc{Scl-Finetune}\\{\scriptsize Acc:$00.00\pm 0.00$}} & \hspace{-0.2in} \hspace{-0.2in} \specialcell{\textsc{Scl-Si}\\{\scriptsize Acc:$00.00\pm 0.00$}} & \hspace{-0.3in} \specialcell{\textsc{Scl-Gss}\\{\scriptsize Acc:$00.00\pm 0.00$}} & \hspace{-0.3in} \specialcell{\textsc{Scl-Der}\\{\scriptsize Acc:$00.00\pm 0.00$}} & \hspace{-0.2in} \specialcell{\textsc{Ucl-Finetune}\\{\scriptsize Acc:$00.00\pm 0.00$}} & \hspace{-0.3in} \specialcell{\textsc{Ucl-Si}\\{\scriptsize Acc:$00.00\pm 0.00$}}& \hspace{-0.3in} \specialcell{\textsc{Lump (Ours)}\\{\scriptsize Acc:$00.00\pm 0.00$}}\\
 \end{tabular}}
\end{minipage}
 \begin{minipage}[t]{1.05\linewidth}
 \resizebox{\linewidth}{!}{%
 \begin{tabular}{c cccc ccc}
 \hspace{-0.2in}
\rb{\includegraphics[width=0.13\textwidth]{figures/tinyimg_feat_maps/T1_imaig4_raw_cropped.PNG}}&
\includegraphics[width=0.17\textwidth]{figures/tinyimg_feat_maps/sup_finetune_3_tiny__T1_imgid4_atT19.png} & \hspace{-0.3in}
\includegraphics[width=0.17\textwidth]{figures/tinyimg_feat_maps/sup_si_1_tinyimg__T1_imgid4_atT19.png} & \hspace{-0.3in}
\includegraphics[width=0.17\textwidth]{figures/tinyimg_feat_maps/sup_gss_3__T1_imgid4_atT19.png} & \hspace{-0.3in}
\includegraphics[width=0.17\textwidth]{figures/tinyimg_feat_maps/sup_der_3_tinyimg__T1_imgid4_atT19.png} & \hspace{-0.2in}
\includegraphics[width=0.17\textwidth]{figures/tinyimg_feat_maps/unsup_finetune_1_tinyimg__T1_imgid4_atT19.png} & \hspace{-0.3in}
\includegraphics[width=0.17\textwidth]{tbd.png} & \hspace{-0.3in}
\includegraphics[width=0.17\textwidth]{figures/tinyimg_feat_maps/unsup_mixup_3_0.4_tiny__T1_imgid4_atT19.png} \vspace{-0.1in}\\
 \hspace{-0.2in} \textsc{Lion} ($t_1$) & \specialcell{\textsc{Scl-Finetune}\\{\scriptsize Acc:$00.00\pm 0.00$}} & \hspace{-0.2in} \hspace{-0.2in} \specialcell{\textsc{Scl-Si}\\{\scriptsize Acc:$00.00\pm 0.00$}} & \hspace{-0.3in} \specialcell{\textsc{Scl-Gss}\\{\scriptsize Acc:$00.00\pm 0.00$}} & \hspace{-0.3in} \specialcell{\textsc{Scl-Der}\\{\scriptsize Acc:$00.00\pm 0.00$}} & \hspace{-0.2in} \specialcell{\textsc{Ucl-Finetune}\\{\scriptsize Acc:$00.00\pm 0.00$}} & \hspace{-0.3in} \specialcell{\textsc{Ucl-Si}\\{\scriptsize Acc:$00.00\pm 0.00$}}& \hspace{-0.3in} \specialcell{\textsc{Lump (Ours)}\\{\scriptsize Acc:$00.00\pm 0.00$}}\\
 \end{tabular}}
 \end{minipage}
  \begin{minipage}[t]{1.05\linewidth}
 \resizebox{\linewidth}{!}{%
 \begin{tabular}{c cccc ccc}
 \hspace{-0.2in}
 \rb{\includegraphics[width=0.13\textwidth]{figures/tinyimg_feat_maps/T2_imaig6_raw_cropped.PNG}}&
\includegraphics[width=0.17\textwidth]{figures/tinyimg_feat_maps/sup_finetune_3_tiny__T2_imgid6_atT19.png} & \hspace{-0.3in}
\includegraphics[width=0.17\textwidth]{figures/tinyimg_feat_maps/sup_si_1_tinyimg__T2_imgid6_atT19.png} & \hspace{-0.3in}
\includegraphics[width=0.17\textwidth]{figures/tinyimg_feat_maps/sup_gss_3__T2_imgid6_atT19.png} & \hspace{-0.3in}
\includegraphics[width=0.17\textwidth]{figures/tinyimg_feat_maps/sup_der_3_tinyimg__T2_imgid6_atT19.png} & \hspace{-0.2in}
\includegraphics[width=0.17\textwidth]{figures/tinyimg_feat_maps/unsup_finetune_1_tinyimg__T2_imgid6_atT19.png} & \hspace{-0.3in}
\includegraphics[width=0.17\textwidth]{tbd.png} & \hspace{-0.3in}
\includegraphics[width=0.17\textwidth]{figures/tinyimg_feat_maps/unsup_mixup_3_0.4_tiny__T2_imgid6_atT19.png} \vspace{-0.1in}\\
\hspace{-0.2in} \textsc{Spider} ($t_2$) & \specialcell{\textsc{Scl-Finetune}\\{\scriptsize Acc:$00.00\pm 0.00$}} & \hspace{-0.2in} \hspace{-0.2in} \specialcell{\textsc{Scl-Si}\\{\scriptsize Acc:$00.00\pm 0.00$}} & \hspace{-0.3in} \specialcell{\textsc{Scl-Gss}\\{\scriptsize Acc:$00.00\pm 0.00$}} & \hspace{-0.3in} \specialcell{\textsc{Scl-Der}\\{\scriptsize Acc:$00.00\pm 0.00$}} & \hspace{-0.2in} \specialcell{\textsc{Ucl-Finetune}\\{\scriptsize Acc:$00.00\pm 0.00$}} & \hspace{-0.3in} \specialcell{\textsc{Ucl-Si}\\{\scriptsize Acc:$00.00\pm 0.00$}}& \hspace{-0.3in} \specialcell{\textsc{Lump (Ours)}\\{\scriptsize Acc:$00.00\pm 0.00$}}\\
 \end{tabular}}
 \end{minipage}
\begin{minipage}[t]{1.05\linewidth}
\resizebox{\linewidth}{!}{%
\begin{tabular}{c cccc ccc}
\hspace{-0.2in}
\rb{\includegraphics[width=0.13\textwidth]{figures/tinyimg_feat_maps/T10_imaig1_raw_cropped.PNG}}&
\includegraphics[width=0.17\textwidth]{figures/tinyimg_feat_maps/sup_finetune_3_tiny__T10_imgid1_atT19.png} & \hspace{-0.3in}
\includegraphics[width=0.17\textwidth]{figures/tinyimg_feat_maps/sup_si_1_tinyimg__T10_imgid1_atT19.png} & \hspace{-0.3in}
\includegraphics[width=0.17\textwidth]{figures/tinyimg_feat_maps/sup_gss_3__T10_imgid1_atT19.png} & \hspace{-0.3in}
\includegraphics[width=0.17\textwidth]{figures/tinyimg_feat_maps/sup_der_3_tinyimg__T10_imgid1_atT19.png} & \hspace{-0.2in}
\includegraphics[width=0.17\textwidth]{figures/tinyimg_feat_maps/unsup_finetune_1_tinyimg__T10_imgid1_atT19.png} & \hspace{-0.3in}
\includegraphics[width=0.17\textwidth]{tbd.png} & \hspace{-0.3in}
\includegraphics[width=0.17\textwidth]{figures/tinyimg_feat_maps/unsup_mixup_3_0.4_tiny__T10_imgid1_atT19.png} \vspace{-0.1in}\\
\hspace{-0.2in} {\small \textsc{Doll} ($\mathcal{T}_{10}$)} & \specialcell{\textsc{Scl-Finetune}\\{\scriptsize Acc:$00.00\pm 0.00$}} & \hspace{-0.2in} \hspace{-0.2in} \specialcell{\textsc{Scl-Si}\\{\scriptsize Acc:$00.00\pm 0.00$}} & \hspace{-0.3in} \specialcell{\textsc{Scl-Gss}\\{\scriptsize Acc:$00.00\pm 0.00$}} & \hspace{-0.3in} \specialcell{\textsc{Scl-Der}\\{\scriptsize Acc:$00.00\pm 0.00$}} & \hspace{-0.2in} \specialcell{\textsc{Ucl-Finetune}\\{\scriptsize Acc:$00.00\pm 0.00$}} & \hspace{-0.3in} \specialcell{\textsc{Ucl-Si}\\{\scriptsize Acc:$00.00\pm 0.00$}}& \hspace{-0.3in} \specialcell{\textsc{Lump (Ours)}\\{\scriptsize Acc:$00.00\pm 0.00$}}\\
\end{tabular}}
\vspace{-0.1in}
\captionof{figure}{\small {\bf Visualization of feature maps} for the second block representations learnt by SCL and UCL strategies for Resnet-18 architecture after the completion of continual learning for Split Tiny-Imagenet dataset ($n=20$). The accuracy is the mean across three runs for the corresponding task. \label{fig:appendix:feature_maps_tiny}}
\vspace{-0.15in}
\end{minipage}
\end{figure*}


==> figures/A_loss_landscapes.tex <==
\begin{figure*}[t!]
\begin{minipage}[t]{1.02\linewidth}
\vspace{-0.1in}
\resizebox{\linewidth}{!}{%
\begin{tabular}{cccccc}
\small
\hspace{-0.15in}\rowlegend{~~~~$\mathcal{T}_0$}
    \includegraphics[width=0.15\textwidth]{figures/images/sclfinetune-t0.PNG} & \hspace{-0.15in}
    \includegraphics[width=0.15\textwidth]{figures/images/sclsi-t0.png} & \hspace{-0.15in}
    %\includegraphics[width=0.15\textwidth]{figures/images/sclgss-t0.png} & \hspace{-0.15in}
    \includegraphics[width=0.15\textwidth]{figures/images/sclder-t0.png} & \hspace{-0.15in}
    \includegraphics[width=0.15\textwidth]{figures/images/uclfinetune-t0.png} & \hspace{-0.15in}
    \includegraphics[width=0.15\textwidth]{figures/images/uclsi-t0.png} & \hspace{-0.15in}
    \includegraphics[width=0.15\textwidth]{figures/images/uclmixup-t0.png} \\
 \hspace{-0.15in}\rowlegend{~~~~$\mathcal{T}_{17}$}
     \includegraphics[width=0.15\textwidth]{figures/images/sclfinetune-t17.PNG} & \hspace{-0.15in}
     \includegraphics[width=0.15\textwidth]{figures/images/sclsi-t17.png} & \hspace{-0.15in}
     %\includegraphics[width=0.15\textwidth]{figures/images/sclgss-t17.png} & \hspace{-0.15in}
     \includegraphics[width=0.15\textwidth]{figures/images/sclder-t17.png} & \hspace{-0.15in}
     \includegraphics[width=0.15\textwidth]{figures/images/uclfinetune-t17.png} & \hspace{-0.15in}
     \includegraphics[width=0.15\textwidth]{figures/images/uclsi-t17.png} & \hspace{-0.15in}
     \includegraphics[width=0.15\textwidth]{figures/images/uclmixup-v2-t17.png} \\
 \hspace{-0.15in}\rowlegend{~~~~$\mathcal{T}_{18}$}
     \includegraphics[width=0.15\textwidth]{figures/images/sclfinetune-t18.PNG} & \hspace{-0.15in}
     \includegraphics[width=0.15\textwidth]{figures/images/sclsi-t18.png} & \hspace{-0.15in}
     %\includegraphics[width=0.15\textwidth]{figures/images/sclgss-t18.png} & \hspace{-0.15in}
     \includegraphics[width=0.15\textwidth]{figures/images/sclder-t18.png} & \hspace{-0.15in}
     \includegraphics[width=0.15\textwidth]{figures/images/uclfinetune-t18.png} & \hspace{-0.15in}
     \includegraphics[width=0.15\textwidth]{figures/images/uclsi-t18.png} & \hspace{-0.15in} 
     \includegraphics[width=0.15\textwidth]{figures/images/uclmixup-v2-t18.png} \\
\hspace{-0.15in}\rowlegend{~~~~$\mathcal{T}_{19}$}    
    \includegraphics[width=0.15\textwidth]{figures/images/sclfinetune-t19.PNG} & \hspace{-0.15in}
    \includegraphics[width=0.15\textwidth]{figures/images/sclsi-t19.png} & \hspace{-0.15in}
    %\includegraphics[width=0.15\textwidth]{figures/images/sclgss-t19.png} & \hspace{-0.15in}
    \includegraphics[width=0.15\textwidth]{figures/images/sclder-t19.png} & \hspace{-0.15in}
    \includegraphics[width=0.15\textwidth]{figures/images/uclfinetune-t19.png} & \hspace{-0.15in}
    \includegraphics[width=0.15\textwidth]{figures/images/uclsi-t19.png} & \hspace{-0.15in}
    \includegraphics[width=0.15\textwidth]{figures/images/uclmixup-v2-t19.png} \\
%\vspace{-0.15in}
\hspace{-0.15in}\specialcell{\textsc{Scl-Finetune}\\{\scriptsize Acc:$54.73\pm 0.25$}} & \hspace{-0.15in} \specialcell{\textsc{Scl-Si}\\{\scriptsize Acc: $58.59\pm 0.20$}} & \hspace{-0.15in} \specialcell{\textsc{Scl-Der}\\{\scriptsize Acc: $73.13\pm 0.38$}} & \hspace{-0.15in}
\specialcell{\textsc{Ucl-Finetune}\\{\scriptsize Acc: $70.80\pm 0.40$}} & \hspace{-0.15in} \specialcell{\textsc{Ucl-Si}\\{\scriptsize Acc: $76.39\pm 1.56$}} &  \hspace{-0.15in} 
\specialcell{\textsc{Lump (Ours)}\\{\scriptsize Acc:$ 76.60\pm 2.70$}}\\
\end{tabular}}
\vspace{-0.1in}
\captionof{figure}{\small {\bf Loss landscape visualization} after the completion of training on task $\mathcal{T}_0$ ({\bf top}) and $\mathcal{T}_{17}, \mathcal{T}_{18}$, and $\mathcal{T}_{19}$ ({\bf bottom}) for Split CIFAR-100 dataset on ResNet-18 architecture. \label{fig:appendix:loss_vis}}
\vspace{-0.3in}
\end{minipage}
\end{figure*}


==> figures/A_rebuttal_lowlv_feature_maps1.tex <==
\begin{figure*}[t!]
\begin{minipage}[t]{1.05\linewidth}
\resizebox{\linewidth}{!}{%
\begin{tabular}{c cccc}
\begin{tabular}{c}     
    \textsc{Raw Images}\\{$\mathcal{T}_0,~\mathcal{T}_1,~\mathcal{T}_2,~\mathcal{T}_{13}$\\~\\~\\~\\~\\~\\~}
\end{tabular}&
\includegraphics[width=0.20\textwidth]{figures/images/T0_imgid0_augmented_raw_cropped.png}&
\includegraphics[width=0.20\textwidth]{figures/images/T1_imgid0_augmented_raw_cropped.png}&
\includegraphics[width=0.20\textwidth]{figures/images/T2_imgid5_raw_cropped.PNG}&
\includegraphics[width=0.20\textwidth]{figures/images/T13_imgid3_augmented_raw_cropped.PNG} \vspace{-0.35in}\\
\begin{tabular}{c}
\textsc{Scl-Finetune}\\Acc:$61.08\pm 0.04$\\~\\~\\~\\~\\~\\~\\~\\~
\end{tabular}&
\includegraphics[width=0.25\textwidth]{figures/rebuttal/sup_finetune_3_c100__T0_imgid0_atT19.png} &
\includegraphics[width=0.25\textwidth]{figures/rebuttal/sup_finetune_3_c100__T1_imgid0_atT19.png} &
\includegraphics[width=0.25\textwidth]{figures/rebuttal/sup_finetune_3_c100__T2_imgid5_atT19.png} &
\includegraphics[width=0.25\textwidth]{figures/rebuttal/sup_finetune_3_c100__T13_imgid3_atT19.png} \vspace{-0.85in}\\
\begin{tabular}{c}
\textsc{Scl-Si}\\ Acc:$63.58\pm 0.37$\\~\\~\\~\\~\\~\\~\\~\\~
\end{tabular}&
\includegraphics[width=0.25\textwidth]{figures/rebuttal/scl_cifar100_si_0p1__T0_imgid0_atT19.png} &
\includegraphics[width=0.25\textwidth]{figures/rebuttal/scl_cifar100_si_0p1__T1_imgid0_atT19.png} &
\includegraphics[width=0.25\textwidth]{figures/rebuttal/scl_cifar100_si_0p1__T2_imgid5_atT19.png} &
\includegraphics[width=0.25\textwidth]{figures/rebuttal/scl_cifar100_si_0p1__T13_imgid3_atT19.png} \vspace{-0.85in}\\
\begin{tabular}{c}
\textsc{Scl-Gss}\\Acc:$70.78\pm 1.67$ \\~\\~\\~\\~\\~\\~\\~\\~
\end{tabular}&
\includegraphics[width=0.25\textwidth]{figures/rebuttal/sup_gss_3__T0_imgid0_atT19.png} &
\includegraphics[width=0.25\textwidth]{figures/rebuttal/sup_gss_3__T1_imgid0_atT19.png} &
\includegraphics[width=0.25\textwidth]{figures/rebuttal/sup_gss_3__T2_imgid5_atT19.png} &
\includegraphics[width=0.25\textwidth]{figures/rebuttal/sup_gss_3__T13_imgid3_atT19.png} \vspace{-0.85in}\\
\begin{tabular}{c}
\textsc{Scl-Der}\\ Acc:$79.52\pm 1.88$\\~\\~\\~\\~\\~\\~\\~\\~
\end{tabular}&
\includegraphics[width=0.25\textwidth]{figures/rebuttal/sup_der_3_c100__T0_imgid0_atT19.png} &
\includegraphics[width=0.25\textwidth]{figures/rebuttal/sup_der_3_c100__T1_imgid0_atT19.png} &
\includegraphics[width=0.25\textwidth]{figures/rebuttal/sup_der_3_c100__T2_imgid5_atT19.png} &
\includegraphics[width=0.25\textwidth]{figures/rebuttal/sup_der_3_c100__T13_imgid3_atT19.png} \vspace{-0.85in}\\
\begin{tabular}{c}
\textsc{Ucl-Finetune}\\Acc:$75.42\pm 0.78$\\~\\~\\~\\~\\~\\~\\~\\~
\end{tabular}&
\includegraphics[width=0.25\textwidth]{figures/rebuttal/unsup_finetune_3_c100__T0_imgid0_atT19.png} &
\includegraphics[width=0.25\textwidth]{figures/rebuttal/unsup_finetune_3_c100__T1_imgid0_atT19.png} &
\includegraphics[width=0.25\textwidth]{figures/rebuttal/unsup_finetune_3_c100__T2_imgid5_atT19.png} &
\includegraphics[width=0.25\textwidth]{figures/rebuttal/unsup_finetune_3_c100__T13_imgid3_atT19.png} \vspace{-0.85in}\\
\begin{tabular}{c}
\textsc{Ucl-Si}\\Acc:$80.08\pm 1.30$\\~\\~\\~\\~\\~\\~\\~\\~
\end{tabular}&\includegraphics[width=0.25\textwidth]{figures/rebuttal/ucl_cifar100_si_100p0__T0_imgid0_atT19.png} &
\includegraphics[width=0.25\textwidth]{figures/rebuttal/ucl_cifar100_si_100p0__T1_imgid0_atT19.png} &
\includegraphics[width=0.25\textwidth]{figures/rebuttal/ucl_cifar100_si_100p0__T2_imgid5_atT19.png} &
\includegraphics[width=0.25\textwidth]{figures/rebuttal/ucl_cifar100_si_100p0__T13_imgid3_atT19.png} \vspace{-0.85in}\\
\begin{tabular}{c}
\textsc{Lump (Ours)}\\Acc:$82.30\pm 1.35$\\~\\~\\~\\~\\~\\~\\~\\~
\end{tabular}&
\includegraphics[width=0.25\textwidth]{figures/rebuttal/ucl_cifar100_mixup_1p0__T0_imgid0_blockid2_atT19.png} &
\includegraphics[width=0.25\textwidth]{figures/rebuttal/ucl_cifar100_mixup_1p0__T1_imgid0_blockid2_atT19.png} &
\includegraphics[width=0.25\textwidth]{figures/rebuttal/ucl_cifar100_mixup_1p0__T2_imgid5_blockid2_atT19.png} &
\includegraphics[width=0.25\textwidth]{figures/rebuttal/ucl_cifar100_mixup_1p0__T13_imgid3_blockid2_atT19.png} \vspace{-0.85in} \\
\end{tabular}}
\captionof{figure}{\small {\bf Visualization of feature maps} for the third block representations learnt by SCL and UCL strategies (with Simsiam) for Resnet-18 architecture after the completion of continual learning for Split CIFAR-100 dataset ($n=20$). The accuracy is the mean across three runs for the corresponding task. \label{fig:appendix:lowlv_feature_maps}}
\vspace{-0.15in}
\end{minipage}
\label{fig:appendix:lowlv_visualize}
\end{figure*}

==> math_commands.tex <==
\usepackage{xcolor}
\usepackage{amsmath,amsfonts,amssymb, amsthm}

%\newenvironment{proof}{\noindent{\bf Proof}\hspace*{1em}}{\qed\bigskip}
\newenvironment{proof-sketch}{\noindent{\bf Sketch of Proof}\hspace*{1em}}{\qed\bigskip}
\newenvironment{proof-idea}{\noindent{\bf Proof Idea}\hspace*{1em}}{\qed\bigskip}
\newenvironment{proof-of-lemma}[1]{\noindent{\bf Proof of Lemma #1}\hspace*{1em}}{\qed\bigskip}
\newenvironment{proof-attempt}{\noindent{\bf Proof Attempt}\hspace*{1em}}{\qed\bigskip}
\newenvironment{proofof}[1]{\noindent{\bf Proof}
of #1:\hspace*{1em}}{\qed\bigskip}
\newenvironment{remark}{\noindent{\bf Remark}\hspace*{1em}}{\bigskip}

% Complex \xxx for making notes of things to do.  Use \xxx{...} for general
% notes, and \xxx[who]{...} if you want to blame someone in particular.
% Puts text in brackets and in bold font, and normally adds a marginpar
% with the text ``xxx'' so that it is easy to find.  On the other hand, if
% the comment is in a minipage, figure, or caption, the xxx goes in the text,
% because marginpars are not possible in these situations.
{\makeatletter
 \gdef\xxxmark{%
   \expandafter\ifx\csname @mpargs\endcsname\relax % in minipage?
     \expandafter\ifx\csname @captype\endcsname\relax % in figure/caption?
       \marginpar{\textcolor{red}{xxx~}}% not in a caption or minipage, can use marginpar
     \else
       \textcolor{red}{xxx~}% notice trailing space
     \fi
   \else
     \textcolor{red}{xxx~}% notice trailing space
   \fi}
 \gdef\xxx{\@ifnextchar[\xxx@lab\xxx@nolab}
 \long\gdef\xxx@lab[#1]#2{{\bf [\xxxmark \textcolor{red}{#2} ---{\sc #1}]}}
 \long\gdef\xxx@nolab#1{{\bf [\xxxmark \textcolor{red}{#1}]}}
}

%\usepackage[T1]{fontenc}
%\usepackage{fourier}
%\DeclareSymbolFont{calletters}{OMS}{cmsy}{m}{n}
%\DeclareSymbolFontAlphabet{\mathcal}{calletters}

\newcommand{\concat}{\mathbin{||}}
\newcommand{\protocol}{\mathbb{P}}

%fields and groups
\newcommand{\F}{\mathbb{F}}
\newcommand{\Fp}{\F_p}
\newcommand{\Fq}{\F_q}
\newcommand{\Ftwo}{\F_2}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\T}{\mathbb{T}}
\newcommand{\Qbar}{\overline{\Q}}
\newcommand{\G}{\mathbb{G}}
\newcommand{\Vs}{\mathbb{V}}
\newcommand{\Fbar}{\overline{\mathbb{F}}}

\DeclareMathOperator*{\Exp}{\mathbb{E}}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\sgn}{sgn}
\DeclareMathOperator*{\pruned}{pruned}
\DeclareMathOperator*{\proj}{proj}
%vectors, etc.
\newcommand{\av}{\mathbf{a}} \newcommand{\cv}{\mathbf{c}}
%\newcommand{\dv}{\mathbf{d}} \newcommand{\ev}{\mathbf{e}}
\newcommand{\rv}{\mathbf{r}} \newcommand{\sv}{\mathbf{s}}
\newcommand{\tv}{\mathbf{t}} \newcommand{\uv}{\mathbf{u}}
\newcommand{\vv}{\mathbf{v}} \newcommand{\wv}{\mathbf{w}}
\newcommand{\xv}{\mathbf{x}} \newcommand{\yv}{\mathbf{y}}
\newcommand{\zv}{\mathbf{z}} \newcommand{\zerov}{\mathbf{0}}
\renewcommand{\AA}{\mathbf{A}} \newcommand{\BB}{\mathbf{B}}
\newcommand{\CC}{\mathbf{C}} \newcommand{\FF}{\mathbf{F}}
\newcommand{\MM}{\mathbf{M}} \newcommand{\RR}{\mathbf{R}}
\renewcommand{\SS}{\mathbf{S}} \newcommand{\TT}{\mathbf{T}}
\newcommand{\UU}{\mathbf{U}} \newcommand{\XX}{\mathbf{X}}
\newcommand{\YY}{\mathbf{Y}} \newcommand{\KK}{\mathbf{K}}
\newcommand{\A}{\mathcal{A}} \newcommand{\B}{\mathcal{B}}
\newcommand{\dash}{\mbox{---}}
\renewcommand{\O}{\mathcal{O}}
%\newcommand{\qq}{\mathfrak{q}}
\newcommand{\QQ}{\mathfrak{Q}}
\newcommand{\ZQ}{\Z_{q}}

\newcommand{\vk}{\mathbf{k}}
%\newcommand{\vu}{\mathbf{u}}

\newcommand{\todo}[1]{\noindent {\color{blue} {\footnotesize {\bf TODO}:~{#1}}}}

\newcommand{\mr}[1]{\ensuremath{\mathrm{{#1}}}}
\newcommand{\la}{\ensuremath{\leftarrow}}
\newcommand{\ra}{\ensuremath{\rightarrow}}
\newcommand{\ala}{\ensuremath{\ \la\ }}
\newcommand{\ara}{\ensuremath{\ \ra\ }}
\newcommand{\rf}{\ensuremath{\overset{\$}{\la}}}

\newcommand{\calA}{\ensuremath{\mathcal{A}}}
\newcommand{\calB}{\ensuremath{\mathcal{B}}}
\newcommand{\calC}{\ensuremath{\mathcal{C}}}
\newcommand{\calD}{\ensuremath{\mathcal{D}}}
\newcommand{\calE}{\ensuremath{\mathcal{E}}}
\newcommand{\calF}{\ensuremath{\mathcal{F}}}
\newcommand{\calG}{\ensuremath{\mathcal{G}}}
\newcommand{\calH}{\ensuremath{\mathcal{H}}}
\newcommand{\calI}{\ensuremath{\mathcal{I}}}
\newcommand{\calJ}{\ensuremath{\mathcal{J}}}
\newcommand{\calK}{\ensuremath{\mathcal{K}}}
\newcommand{\calL}{\ensuremath{\mathcal{L}}}
\newcommand{\calM}{\ensuremath{\mathcal{M}}}
\newcommand{\calN}{\ensuremath{\mathcal{N}}}
\newcommand{\calO}{\ensuremath{\mathcal{O}}}
\newcommand{\calP}{\ensuremath{\mathcal{P}}}
\newcommand{\calQ}{\ensuremath{\mathcal{Q}}}
\newcommand{\calR}{\ensuremath{\mathcal{R}}}
\newcommand{\calS}{\ensuremath{\mathcal{S}}}
\newcommand{\calT}{\ensuremath{\mathcal{T}}}
\newcommand{\calU}{\ensuremath{\mathcal{U}}}
\newcommand{\calV}{\ensuremath{\mathcal{V}}}
\newcommand{\calW}{\ensuremath{\mathcal{W}}}
\newcommand{\calX}{\ensuremath{\mathcal{X}}}
\newcommand{\calY}{\ensuremath{\mathcal{Y}}}
\newcommand{\calZ}{\ensuremath{\mathcal{Z}}}

% -- bold math symbols, for some reason --
\newcommand{\boldalpha}{\ensuremath{\boldsymbol{\alpha}}}
\newcommand{\boldchi}{\ensuremath{\boldsymbol{\chi}}}
\newcommand{\boldtau}{\ensuremath{{\boldsymbol{\tau}}}}
\newcommand{\boldstar}{\ensuremath{\mathbf{*}}}
\newcommand{\bolda}{\ensuremath{\mathbf{a}}}
\newcommand{\boldb}{\ensuremath{\mathbf{b}}}
\newcommand{\boldc}{\ensuremath{\mathbf{c}}}
\newcommand{\boldd}{\ensuremath{\mathbf{d}}}
\newcommand{\bolde}{\ensuremath{\mathbf{e}}}
\newcommand{\boldf}{\ensuremath{\mathbf{f}}}
\newcommand{\boldg}{\ensuremath{\mathbf{g}}}
\newcommand{\boldh}{\ensuremath{\mathbf{h}}}
\newcommand{\boldi}{\ensuremath{\mathbf{i}}}
\newcommand{\boldj}{\ensuremath{\mathbf{j}}}
\newcommand{\boldk}{\ensuremath{\mathbf{k}}}
\newcommand{\boldl}{\ensuremath{\mathbf{l}}}
\newcommand{\boldm}{\ensuremath{\mathbf{m}}}
\newcommand{\boldn}{\ensuremath{\mathbf{n}}}
\newcommand{\boldo}{\ensuremath{\mathbf{o}}}
\newcommand{\boldp}{\ensuremath{\mathbf{p}}}
\newcommand{\boldq}{\ensuremath{\mathbf{q}}}
\newcommand{\boldr}{\ensuremath{\mathbf{r}}}
\newcommand{\bolds}{\ensuremath{\mathbf{s}}}
\newcommand{\boldt}{\ensuremath{\mathbf{t}}}
\newcommand{\boldu}{\ensuremath{\mathbf{u}}}
\newcommand{\boldv}{\ensuremath{\mathbf{v}}}
\newcommand{\boldw}{\ensuremath{\mathbf{w}}}
\newcommand{\boldx}{{\ensuremath{\mathbf{x}}}}
\newcommand{\boldy}{\ensuremath{\mathbf{y}}}
\newcommand{\boldz}{\ensuremath{\mathbf{z}}}
\newcommand{\boldzero}{\ensuremath{\boldsymbol{0}}}
\newcommand{\boldone}{\ensuremath{\boldsymbol{1}}}
\newcommand{\boldpi}{\ensuremath{\boldsymbol{\pi}}}
\newcommand{\boldPi}{\ensuremath{\boldsymbol{\Pi}}}

% -- bold italic math symbols, for some reason --
\newcommand{\boldia}{\ensuremath{\boldsymbol{a}}}
\newcommand{\boldib}{\ensuremath{\boldsymbol{b}}}
\newcommand{\boldic}{\ensuremath{\boldsymbol{c}}}
\newcommand{\boldid}{\ensuremath{\boldsymbol{d}}}
\newcommand{\boldie}{\ensuremath{\boldsymbol{e}}}
\newcommand{\boldif}{\ensuremath{\boldsymbol{f}}}
\newcommand{\boldig}{\ensuremath{\boldsymbol{g}}}
\newcommand{\boldih}{\ensuremath{\boldsymbol{h}}}
\newcommand{\boldii}{\ensuremath{\boldsymbol{i}}}
\newcommand{\boldij}{\ensuremath{\boldsymbol{j}}}
\newcommand{\boldik}{\ensuremath{\boldsymbol{k}}}
\newcommand{\boldil}{\ensuremath{\boldsymbol{l}}}
\newcommand{\boldim}{\ensuremath{\boldsymbol{m}}}
\newcommand{\boldin}{\ensuremath{\boldsymbol{n}}}
\newcommand{\boldio}{\ensuremath{\boldsymbol{o}}}
\newcommand{\boldip}{\ensuremath{\boldsymbol{p}}}
\newcommand{\boldiq}{\ensuremath{\boldsymbol{q}}}
\newcommand{\boldir}{\ensuremath{\boldsymbol{r}}}
\newcommand{\boldis}{\ensuremath{\boldsymbol{s}}}
\newcommand{\boldit}{\ensuremath{\boldsymbol{t}}}
\newcommand{\boldiu}{\ensuremath{\boldsymbol{u}}}
\newcommand{\boldiv}{\ensuremath{\boldsymbol{v}}}
\newcommand{\boldiw}{\ensuremath{\boldsymbol{w}}}
\newcommand{\boldix}{\ensuremath{\boldsymbol{x}}}
\newcommand{\boldiy}{\ensuremath{\boldsymbol{y}}}
\newcommand{\boldiz}{\ensuremath{\boldsymbol{z}}}

\newcommand{\transpose}[1]{\ensuremath{{#1}^{\intercal}}}

\newcommand{\boldA}{\ensuremath{\mathbf{A}}}
\newcommand{\boldB}{\ensuremath{\mathbf{B}}}
\newcommand{\boldC}{\ensuremath{\mathbf{C}}}
\newcommand{\boldD}{\ensuremath{\mathbf{D}}}
\newcommand{\boldE}{\ensuremath{\mathbf{E}}}
\newcommand{\boldF}{\ensuremath{\mathbf{F}}}
\newcommand{\boldG}{\ensuremath{\mathbf{G}}}
\newcommand{\boldH}{\ensuremath{\mathbf{H}}}
\newcommand{\boldI}{\ensuremath{\mathbf{I}}}
\newcommand{\boldJ}{\ensuremath{\mathbf{J}}}
\newcommand{\boldK}{\ensuremath{\mathbf{K}}}
\newcommand{\boldL}{\ensuremath{\mathbf{L}}}
\newcommand{\boldM}{\ensuremath{\mathbf{M}}}
\newcommand{\boldN}{\ensuremath{\mathbf{N}}}
\newcommand{\boldO}{\ensuremath{\mathbf{O}}}
\newcommand{\boldP}{\ensuremath{\mathbf{P}}}
\newcommand{\boldQ}{\ensuremath{\mathbf{Q}}}
\newcommand{\boldR}{\ensuremath{\mathbf{R}}}
\newcommand{\boldS}{\ensuremath{\mathbf{S}}}
\newcommand{\boldT}{\ensuremath{\mathbf{T}}}
\newcommand{\boldU}{\ensuremath{\mathbf{U}}}
\newcommand{\boldV}{\ensuremath{\mathbf{V}}}
\newcommand{\boldW}{\ensuremath{\mathbf{W}}}
\newcommand{\boldX}{\ensuremath{\mathbf{X}}}
\newcommand{\boldY}{\ensuremath{\mathbf{Y}}}
\newcommand{\boldZ}{\ensuremath{\mathbf{Z}}}

\newcommand{\deq}{\mathrel{\mathop:}=}
\newcommand{\zo}{\ensuremath{\{0,1\}}} % bits
\newcommand{\zon}{\ensuremath{\{0,1\}^n}} % bits

% Theorem definitions

\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{definition}
\newtheorem*{claims}{Claim}
\newtheorem{defn}[theorem]{Definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{myremark}[theorem]{Remark}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{construction}[theorem]{Construction}

%% custom macros

\newcommand{\esm}[1]{\ensuremath{#1}}
\newcommand{\ms}[1]{\esm{\mathsf{#1}}}

\newcommand{\prg}{\ms{PRG}}
\newcommand{\prf}{\ms{PRF}}
\newcommand{\prp}{\ms{PRP}}
\newcommand{\enc}{\ms{Enc}}
\newcommand{\compute}{\ms{Compute}}
\newcommand{\verify}{\ms{Verify}}

\newcommand{\poly}{\esm{\mr{poly}}}
\newcommand{\polylog}{\operatorname{polylog}}
\newcommand{\negl}{\esm{\mr{negl}}}

\newcommand{\ord}[1]{\esm{{#1}^{\mr{th}}}}

\newcommand{\hyb}{\ms{Hyb}}
\newcommand{\Funs}{\ms{Funs}}
\newcommand{\getsr}{\xleftarrow{\textsc{r}}}
\newcommand{\Unif}{\ms{Unif}}

\newcommand{\appc}{\stackrel{c}{\approx}}
\newcommand{\apps}{\stackrel{s}{\approx}}
%\newcommand{\abs}[1]{\left| #1 \right|}

\newcommand{\classP}{\ms{P}}
\newcommand{\classBPP}{\ms{BPP}}
\newcommand{\classNP}{\ms{NP}}
\newcommand{\Ppoly}{\ms{P}/\ms{poly}}
\newcommand{\NCone}{\ms{NC^1}}

\newcommand{\round}[1]{\left\lfloor #1 \right\rceil}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\iprod}[1]{\left\langle #1 \right\rangle}
%\newcommand{\norm}[1]{\left\| #1 \right\|}
\newcommand{\set}[1]{\left\{ #1 \right\}}

\newcommand{\Zp}{\Z_p}
\newcommand{\Zq}{\Z_q}

\DeclareMathOperator{\Ber}{Ber}
\DeclareMathOperator{\gammadist}{gamma}
\DeclareMathOperator{\betadist}{beta}
\DeclareMathOperator{\Dir}{Dir}
\DeclareMathOperator{\cat}{cat}
\DeclareMathOperator{\expon}{expon}
\DeclareMathOperator{\unif}{unif}
\DeclareMathOperator{\KL}{D_{KL}}
\DeclareMathOperator{\sgm}{sgm}
\DeclareMathOperator{\hsgm}{hsgm}
\DeclareMathOperator{\Frob}{{F}}
\DeclareMathOperator{\diag}{{diag}}

\newcommand{\subind}[2]{{#1}^{(#2)}}

\newcommand{\eqq}{\stackrel{?}{=}}

\newcommand{\Otilde}{\widetilde{O}}

\newcommand{\hc}{\ms{hc}}

\newcommand{\xstar}{x^*}
\newcommand{\ystar}{y^*}

\newcommand{\DDHAdv}{\ms{DDHAdv}}
\newcommand{\PRFAdv}{\ms{PRFAdv}}
\newcommand{\SCPRFAdv}{\ms{SC\hbox{-}PRFAdv}}

\newcommand{\ct}{\ms{ct}}

\newcommand{\view}{\ms{view}_{P,V^*}}
\newcommand{\viewHonest}{\ms{view}_{P,V}}
\newcommand{\Sim}{\calS}

\newcommand{\Am}{\mathbf{A}}

\newcommand{\SIS}{\ms{SIS}}
\newcommand{\ISIS}{\ms{ISIS}}
\newcommand{\LWE}{\ms{LWE}}
\newcommand{\mLWE}{\ms{MatrixLWE}}

\newcommand{\Sm}{\mathbf{S}}
\newcommand{\Em}{\mathbf{E}}
\newcommand{\Um}{\mathbf{U}}

\newcommand{\LWEadv}{\ms{LWEAdv}}
\newcommand{\mLWEadv}{\ms{MatrixLWEAdv}}
\newcommand{\SISadv}{\ms{SISAdv}}
\newcommand{\ISISadv}{\ms{ISISAdv}}

\newcommand{\bv}{\mathbf{b}}
\newcommand{\Bm}{\mathbf{B}}
\newcommand{\Rm}{\mathbf{R}}

\newcommand{\pro}[1]{\langle #1 \rangle}
\newcommand{\Comm}{\ms{Commit}}
\newcommand{\cSAT}{\ms{circuit}\text{-}\ms{SAT}}

\newcommand{\sk}{\ms{sk}}

\newcommand{\hin}{h_{\text{in}}}
\newcommand{\hout}{h_{\text{out}}}
\newcommand{\chin}{c_{\text{in}}}
\newcommand{\chout}{c_{\text{out}}}
\newcommand{\patches}{\texttt{patches}}
\newcommand{\FP}{\texttt{FP}}
\newcommand{\conv}{\texttt{Conv}}

\newcommand{\proctrust}{\calP_{T}}
\newcommand{\procuntrust}{\calP_{U}}

\newenvironment{myitemize}
{\begin{itemize}[leftmargin=5.5mm, itemsep=2pt, topsep=0pt]}
	{\end{itemize}}

\newenvironment{myenumerate}
{\begin{enumerate}[leftmargin=5.5mm, itemsep=1pt, topsep=0pt]}
	{\end{enumerate}}

\renewcommand{\wp}{\ \textnormal{w.p.}\ }

\newcommand{\sign}{\textrm{sign}}
\newcommand{\Bernoulli}[1]{\texttt{Bernoulli}(#1)}
\newcommand{\relu}{\textrm{ReLU}}
\newcommand{\xadv}{x_{\textrm{adv}}}

\newcommand*\diff{\mathop{}\!\mathrm{d}}
\renewcommand{\vec}[1]{\mathbold{#1}}

\newcommand{\Var}{\operatorname{Var}}
\newcommand{\OPT}{\operatorname{OPT}}
